Photoproduction Reactions and Non-Strange Baryon Spectroscopy

We review the last two decades of using photon beams to measure the production of mesons, and in particular the information that can be obtained on the spectrum of light, non-strange baryons. This is a compendium of experimental results, which should be used as a complement to theoretical reviews of the subject. Lists of data sets are given, together with a comprehensive set of references. An indication of the impact of the data is presented with a summary of the results.

==> Photo production reactions and baryon spectroscopy/asymm-config-table.tex <==
% This is a table of all the possible experimental 
% configurations in pseudoscalar meson photoproduction. 
% It may be better to have this as an appendix - DGI

% \begin{landscape}
% \advance\vsize6cm
% \csname @colroom\endcsname=\vsize
% \textheight=\vsize
% \csname @colht\endcsname=\vsize


\begin{longtable}{C{1.5cm} C{1.5cm} C{3.5cm} p{8.5cm} >{(\refstepcounter{subexno}\theexno)} C{1cm}}
\captionsetup{width=.75\textwidth}
\caption{\label{tab:asymmetries} Expressions for asymmetries for different experiments. The definitions of angles are shown in figure \ref{fig:axes}. Configurations are labeled U, C and L for unpolarized, circular and linear polarized photon beams; U, L and T for unpolarized, longitudinal and transverse target polarization. Where degrees of polarization are labelled +ve or -ve, this refers to their direction with respect to an axis: lab $x$, $y$ or $z$ for target polarization; photon beam direction for circular photon polarization. } \\
%\begin{table*}
%\rowcolors{3}{gray!25}{}

% \begin{tabularx}{\textwidth}{C{2cm} C{2cm} C{2cm} R >{(\refstepcounter{exno}\theexno)}C{1cm}} 
\toprule
%\begin{tabularx}{\textwidth}{*{4}{X}}    \toprule
\multicolumn{3}{c}{\emph{Configuration}} &  
\hfil\multirow{2}[8]{*}{\emph{Asymmetry formula, $A_\sigma$}}\hfill \\
\cmidrule(lr){1-3}
Beam & Target & Settings &   \\ 

\endfirsthead
\midrule


Beam & Target & Settings &  \hfil\emph{Asymmetry formula, $A_\sigma$}\hfill \\
\midrule
\endhead

\multicolumn{5}{r}{\emph{Continued on next page}}
\endfoot
\endlastfoot

\midrule 
\addlinespace[0.5em]
%--------------------------------------------------------------------------
\multirow{2}*[-1.5em]{U}  
    & L
    & $\tarpol_z\;+$ve; $\tarpol_z\;-$ve      
    & $\dfrac{\tarpol_z \left(\obs{L_{x^\prime}} \recpol_{x^\prime} + \obs{L_{z^\prime}} \recpol_{z^\prime} \right)}{1 + \obs{P} \recpol_{y^\prime}}
                       $
    					 & \label{a:row1} \\
\addlinespace[1.0em]                         

    & T       
    & $\beta = 0;\;\beta=\pi$      
    & 
    $\begin{aligned}
    \dfrac{ \tarpol_T}
    {1 + \obs{P} \recpol_{y^\prime}}
    & \left\{ 
    \left( \obs{T_{x^\prime}} \recpol_{x^\prime} +   \obs{T_{z^\prime}} \recpol_{z^\prime} \right) \cos \phi
        \right. \\
    & \left. \enspace -
    \left( \obs{\Sigma} \recpol_{y^\prime} + \obs{T} 
       \right) \sin \phi 
    \right\}
    \end{aligned}$
                         & \label{a:row2} \\
\addlinespace[0.5em]
\midrule 
\addlinespace[0.5em]
%--------------------------------------------------------------------------
%\pagebreak
\multirow{3}*[-3.45em]{C}    
    & U    
    & $\circpol\;+$ve; $\circpol\;-$ve      
    & $\dfrac{\circpol \left(\obs{C_{x^\prime}} \recpol_{x^\prime} + \obs{C_{z^\prime}} \recpol_{z^\prime} \right)}{1 + \obs{P} \recpol_{y^\prime}}$
    & \label{a:row3} \\

\addlinespace[1.0em]

    & L
    & ($\circpol\;+$ve, $\tarpol_z\;+$ve |
      $\circpol\;-$ve, $\tarpol_z\;-$ve); 
      ($\circpol\;+$ve, $\tarpol_z\;-$ve |
      $\circpol\;-$ve, $\tarpol_z\;+$ve) 
    & $\dfrac{\circpol \tarpol_z \left(\obs{E} + \obs{H} \recpol_{y^\prime} \right)}{1 + \obs{P} \recpol_{y^\prime}}$
    & \label{a:row4} \\ 
    
\addlinespace[1.0em]
    
    & T
    & ($\circpol\;+$ve, $\beta=0$ |
      $\circpol\;-$ve, $\beta=\pi$); 
      ($\circpol\;+$ve, $\beta=0$ |
      $\circpol\;-$ve, $\beta=\pi$)   
    & 
    $\begin{aligned}
    \dfrac{ \circpol \tarpol_T}
    {1 + \obs{P} \recpol_{y^\prime}}
    & \left\{ 
    \left(  \obs{F}  + \obs{G} \recpol_{y^\prime} \right) 
    \cos \phi
        \right. \\
    & \left. \enspace -
    \left( \obs{O_{x^\prime}} \recpol_{z^\prime} - \obs{O_{z^\prime}} \recpol_{x^\prime}
       \right)
    \sin \phi 
    \right\}
    \end{aligned}$
    & \label{a:row5}\\ %\pagebreak
    \addlinespace[0.5em]
\midrule 
\addlinespace[0.5em]

%--------------------------------------------------------------------------
\pagebreak
\addlinespace[0.5em]
\multirow{3}*[-4.2em]{L}    
    & U    
    & $\alpha=0$; $\alpha=\frac{\pi}{2}$      
    & 
    $\begin{aligned}
    \dfrac{ - \linpol }
    {1 + \obs{P} \recpol_{y^\prime}}
    & \left\{ 
    \left(  \obs{\Sigma}  + \obs{T} \recpol_{y^\prime} \right) 
    \cos 2 \phi
        \right. \\
    & \left. \enspace +
    \left( \obs{O_{x^\prime}} \recpol_{x^\prime} -      
    \obs{O_{z^\prime}} \recpol_{z^\prime}
       \right) 
    \sin 2 \phi
    \right\}
    \end{aligned}$
    & \label{a:row6}\\ 
\addlinespace[1.0em]
    & L
    & ($\alpha=0$, $\tarpol_z\;+$ve |
      $\alpha=\frac{\pi}{2}$, $\tarpol_z\;-$ve); 
      ($\alpha=0$, $\tarpol_z\;-$ve |
      $\alpha=\frac{\pi}{2}$, $\tarpol_z\;+$ve)      
    & 
    $\begin{aligned}
    \dfrac{ - \linpol \tarpol_z}
    {1 + \obs{P} \recpol_{y^\prime}}
    & \left\{ 
    \left(  \obs{T_{x^\prime}} \recpol_{z^\prime} - \obs{T_{z^\prime}} \recpol_{x^\prime} \right) 
    \cos 2 \phi
        \right. \\
    & \left. \enspace +
    \left( \obs{F} \recpol_{y^\prime} + \obs{G}
       \right) 
    \sin 2 \phi
    \right\}
    \end{aligned}$
                        & \label{a:row7} \\ 
                        
    \addlinespace[1.0em]
    
    & T
    & ($\alpha=0$, $\beta=0$ |
      $\alpha=\frac{\pi}{2}$, $\beta=\pi$); 
      ($\alpha=0$, $\beta=0$ |
      $\alpha=\frac{\pi}{2}$, $\beta=\pi$)      
    & $\begin{aligned}
    \dfrac{ \linpol \tarpol_T}
    {1 + \obs{P} \recpol_{y^\prime}}
    & \left\{ 
    \left( \recpol_{y^\prime} + \obs{P}  \right) 
    \sin\phi \cos 2 \phi 
    \right. \\
    & +
     \left( \obs{L_{x^\prime}} \recpol_{z^\prime} - \obs{L_{z^\prime}} \recpol_{x^\prime}\right) 
    \cos\phi \cos 2 \phi 
    \\
    & +
     \left( \obs{C_{x^\prime}} \recpol_{z^\prime} - \obs{C_{z^\prime}} \recpol_{x^\prime} \right) 
    \sin\phi \sin 2 \phi 
    \\    
    & \left. +
     \left( \obs{E} \recpol_{y^\prime}  + \obs{H} \right) 
    \cos\phi \sin 2 \phi 
    \right\}
    \end{aligned}
    $
    & \label{a:row8} \\ 
    \addlinespace[0.5em]
\bottomrule %--------------------------------------------------------------------------
%\end{tabularx}
%\end{table*}  


\end{longtable}
% \end{landscape}

==> Photo production reactions and baryon spectroscopy/exp-config-table.tex <==
% This is a table of all the possible experimental 
% configurations in pseudoscalar meson photoproduction. 
% It may be better to have this as an appendix - DGI

% \begin{landscape}
% \advance\vsize6cm
% \csname @colroom\endcsname=\vsize
% \textheight=\vsize
% \csname @colht\endcsname=\vsize


\begin{longtable}{C{2cm} C{2cm} C{1.5cm} p{9.5cm} >{(\refstepcounter{subexno}\theexno)} C{1cm}}
\captionsetup{width=.75\textwidth}
\caption{\label{tab:cross-sections} Expressions for cross sections for different experiments.}\\
%\begin{table*}
%\rowcolors{3}{gray!25}{}

% \begin{tabularx}{\textwidth}{C{2cm} C{2cm} C{2cm} R >{(\refstepcounter{exno}\theexno)}C{1cm}} 
\toprule
%\begin{tabularx}{\textwidth}{*{4}{X}}    \toprule
\multicolumn{3}{c}{\emph{Configuration}} &  
\hfil\multirow{2}[8]{*}{\emph{Cross section formula, $\sigma/\sigma_0$}}\hfill \\
\cmidrule(lr){1-3}
Beam & Target & Recoil &   \\ 

\endfirsthead
\midrule


Beam & Target & Recoil &  \hfil\emph{Cross section formula, $\sigma/\sigma_0$}\hfill \\
\midrule
\endhead

\multicolumn{5}{r}{\emph{Continued on next page}}
\endfoot
\endlastfoot

\midrule 

%--------------------------------------------------------------------------
\multirow{6}*{Unpolarized}    
    & \multirow{2}*{Unpolarized}    
            & N      & 1 & \label{row1}\\  
\cmidrule(r){4-5}
    &       & Y      & $1 + \obs{P} \recpol_{y^\prime}$ & \label{row2} \\
\cmidrule[0.7\cmidrulewidth](lr){3-5}
    & \multirow{2}*{Longitudinal}
            & N     & 1 & \label{row3} \\ 
\cmidrule(r){4-5}
    &       & Y      & $
    					1 + \obs{P} \recpol_{y^\prime} + 
                        \left(
                        \obs{L_{x^\prime}} \recpol_{x^\prime} + \obs{L_{z^\prime}} \recpol_{z^\prime} 
                        \right) \tarpol_z
                       $
    					 & \label{row4}\\
\cmidrule[0.7\cmidrulewidth](lr){3-5}
    & \multirow{2}*{Transverse}
             & N      & $1 + \obs{T} \tarpol_T \sin (\beta -\phi) $ & \label{row5}\\ 
\cmidrule(r){4-5} \addlinespace[0.5em]
    &        & Y      &  
    					
    					 $\begin{aligned}
                         & 1 + \obs{P} \recpol_{y^\prime} 
                         + 
						 \left( 
                         \obs{\Sigma} \recpol_{y^\prime} + \obs{T} 
                         \right) \tarpol_T \sin (\beta -\phi) \\
                         & \enspace +
                         \left( 
                         \obs{T_{x^\prime}} \recpol_{x^\prime} + \obs{T_{z^\prime}} \recpol_{z^\prime} 
                         \right) \tarpol_T \cos (\beta - \phi)
                        \end{aligned}$
                        
                         & \label{row6} \\
\midrule 

%--------------------------------------------------------------------------
%\pagebreak
\multirow{6}*[-4.0em]{Circular}    
    & \multirow{2}*{Unpolarized}    
            & N      & 1 & \label{row7} \\ 
\cmidrule(r){4-5}
    &       & Y      & $
                        1 + \obs{P} \recpol_{y^\prime} +
                        \left(
                        \obs{C_{x^\prime}} \recpol_{x^\prime} + \obs{C_{z^\prime}} \recpol_{z^\prime}
                        \right) \circpol 
                       $
                        & \label{row8} \\
\cmidrule[0.7\cmidrulewidth](lr){3-5}
    & \multirow{2}*{Longitudinal}
            & N      & $ 
                        1 - \obs{E} \circpol \tarpol_y 
                       $ & \label{row9} \\ 
\cmidrule(r){4-5} \addlinespace[0.5em]
    &       & Y      & $ 
    					\begin{aligned}
    					& 1 + \obs{P} \recpol_{y^\prime} + \left(
                        \obs{L_{x^\prime}} \recpol_{x^\prime} + \obs{L_{z^\prime}} \recpol_{z^\prime} 
                        \right) \tarpol_z \\
                        & \enspace + \left\{ 
                        \obs{C_{x^\prime}}  \recpol_{x^\prime} + \obs{C_{z^\prime}} \recpol_{z^\prime} 
                        - \left(
                        \obs{E} + \obs{H} \recpol_{y^\prime} 
                        \right) \tarpol_z 
                        \right\} \circpol
    					\end{aligned}
                       $ 
                        & \label{row10} \\ \addlinespace[0.5em]
\cmidrule[0.7\cmidrulewidth](lr){3-5}
    & \multirow{2}*{Transverse}
             & N      & $
                         1 + \obs{T} \tarpol_T \sin (\beta -\phi) +
                         \obs{F} \circpol \tarpol_T \cos (\beta -\phi)
                        $
                         & \label{row11} \\ 
\cmidrule(r){4-5} \addlinespace[0.5em]
    &        & Y      & $
                         \begin{aligned}
                         & 1 + \obs{P} \recpol_{y^\prime} 
						 + \left( 
                         \obs{\Sigma} \recpol_{y^\prime} + \obs{T} 
                         \right) \tarpol_T \sin (\beta -\phi) \\ 
                         & \enspace + \left( 
                         \obs{T_{x^\prime}} \recpol_{x^\prime} + \obs{T_{z^\prime}} \recpol_{z^\prime} 
                         \right) \tarpol_T \cos (\beta-\phi) \\
                         & \enspace +
                         \left\{
                         \obs{C_{x^\prime}} \recpol_{x^\prime} 
                         + \obs{C_{z^\prime}} \recpol_{z^\prime} 
                         + \left(
                         \obs{F}  + \obs{G} 
                         \recpol_{y^\prime}  \right) \tarpol_T \cos (\beta-\phi) \right.\\
                         & \left. \qquad + \left( 
                         \obs{O_{x^\prime}} \recpol_{z^\prime} - \obs{O_{z^\prime}} \recpol_{x^\prime} 
                         \right) \tarpol_T \sin (\beta-\phi)
                         \right\}\circpol
                         \end{aligned}
                        $
                         & \label{row12}\\ \addlinespace[0.5em]
\midrule 
%--------------------------------------------------------------------------
%\pagebreak
\multirow{6}*[-5.0em]{Linear}    
    & \multirow{2}*{Unpolarized}    
            & N      & $1 - \obs{\Sigma} \linpol \cos 2(\alpha-\phi)$ & \label{row13}\\ 
\cmidrule(r){4-5} \addlinespace[0.5em]
    &       & Y      & 
                       $\begin{aligned}
                       & 1 + \obs{P} \recpol_{y^\prime}  -
                        \left\{
                        \obs{\Sigma} + \obs{T} \recpol_{y^\prime}
                        \right\} \linpol \cos 2(\alpha-\phi) \\
                        & \enspace +
                        \left\{
                        \obs{O_{x^\prime}} \recpol_{x^\prime} + \obs{O_{z^\prime}} \recpol_{z^\prime}
                        \right\} \linpol \sin 2(\alpha-\phi) \end{aligned} 
                       $ 
                        & \label{row14}\\ \addlinespace[0.5em]
\cmidrule[0.7\cmidrulewidth](lr){3-5}
    & \multirow{2}*{Longitudinal}
            & N      &  $1 - \obs{\Sigma} \linpol \cos 2(\alpha-\phi) +
                         \obs{G} \tarpol_y \linpol \sin 2(\alpha-\phi)$& \label{row15}\\ 
\cmidrule(r){4-5} \addlinespace[0.5em]
    &       & Y      & $ \begin{aligned}
                        &1 + \obs{P} \recpol_{y^\prime} + 
                        \left(
                        \obs{L_{x^\prime}} \recpol_{x^\prime} + 
                        \obs{L_{z^\prime}} \recpol_{z^\prime} 
                        \right) \tarpol_z \\
                        & \; - 
                        \left\{
                        \obs{\Sigma} + \obs{T} \recpol_{y^\prime} +   
                        \left(
                        \obs{T_{x^\prime}} \recpol_{z^\prime} - \obs{T_{z^\prime}} \recpol_{x^\prime} 
                        \right) \tarpol_z
                        \right\} \linpol \cos 2(\alpha-\phi) \\
                        & \; +
                        \left\{
                        \left(
                        \obs{F} \recpol_{y^\prime} + \obs{G} 
                        \right) \tarpol_z + 
                        \obs{O_{x^\prime}} \recpol_{x^\prime} + \obs{O_{z^\prime}} \recpol_{z^\prime}
                        \right\} \linpol \sin 2(\alpha-\phi)
                        \end{aligned}
                        $
                        & \label{row16} \\ \nopagebreak \addlinespace[0.5em]
\cmidrule[0.7\cmidrulewidth](lr){3-5} \addlinespace[0.5em]
    & \multirow{2}*[-2.0em]{Transverse}
             & N      & $\begin{aligned}
                         & 1 + \obs{T} \tarpol_T \sin (\beta-\phi) \\
                         & \enspace -
                         \left\{
                         \obs{\Sigma}+ 
                         \obs{P} \tarpol_T \sin(\beta-\phi) 
                         \right\} \linpol \cos 2(\alpha-\phi) \\
                         & \enspace +
                         \obs{H} \tarpol_T \cos(\beta-\phi) \linpol \sin 2(\alpha-\phi)
                         \end{aligned}
                        $
                         & \label{row17} \\ \addlinespace[0.5em]
\cmidrule(r){4-5} \addlinespace[0.5em]
    &        & Y      & $
                         \begin{aligned}
                         & 1 - \linpol \recpol_{y^\prime} \tarpol_T \sin(\beta-\phi) 
                         \cos 2(\alpha-\phi) + \obs{P} \recpol_{y^\prime} \\
                         & \enspace +
                         \left(
                         \obs{T_{x^\prime}} \recpol_{x^\prime} + \obs{T_{z^\prime}} \recpol_{z^\prime}
                         \right) \tarpol_T \cos(\beta-\phi) \\
                         & \enspace + 
                         \left(
                         \obs{\Sigma} \recpol_{y^\prime} + \obs{T}
                         \right) \tarpol_T \sin(\beta-\phi) \\
                         & \enspace -
                         \left\{
                          \obs{\Sigma} 
                         + \obs{T} \recpol_{y^\prime}
                         + \obs{P} \tarpol_T \sin(\beta-\phi) \right. \\
                         & \left. \qquad - \left(
                         \obs{L_{x^\prime}} \recpol_{z^\prime} - \obs{L_{z^\prime}} \recpol_{x^\prime}
                         \right) \tarpol_T \cos(\beta-\phi)
                         \right\} \linpol \cos 2(\alpha-\phi) \\
                         & \enspace +
                         \left\{
                         \obs{O_{x^\prime}} \recpol_{x^\prime} + \obs{O_{z^\prime}} \recpol_{z^\prime} 
                         + \left(
                         \obs{E} \recpol_{y^\prime}  + \obs{H} 
                         \right) \tarpol_T \cos(\beta-\phi) \right. \\
          	             & \left. \qquad - \left(
                         \obs{C_{x^\prime}} \recpol_{z^\prime} - \obs{C_{z^\prime}} \recpol_{x^\prime} 
                         \right) \tarpol_T \sin(\beta-\phi) 
                         \right\} \linpol \sin 2(\alpha-\phi)
                         \end{aligned}
						$
                         & \label{row18} \\ \addlinespace[0.5em]
\bottomrule %--------------------------------------------------------------------------
%\end{tabularx}
%\end{table*}  


\end{longtable}
% \end{landscape}

==> Photo production reactions and baryon spectroscopy/header.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	File: 		header.tex
%	Content:	Formatting and definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Additional LaTeX packages...
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{fancyvrb}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage[latin1]{inputenc}
\usepackage{longtable}
\usepackage{lscape}
\usepackage[fleqn]{mathtools}
\usepackage{lipsum}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{pifont}
\usepackage{siunitx}
\usepackage{tabularx}
\usepackage{units}
\usepackage{caption}
\usepackage{float}
\usepackage{afterpage}

% Unused/conflicted...
%\usepackage[table]{xcolor} 
%\usepackage{mathpazo}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% New definitions...
\def\Journal#1#2#3#4{{#1} {#2} (#4) #3}
\def\EPJA{{\em Eur. Phys. J.} A}
\def\NCA{{\em Nuovo Cimento} A}
\def\PHYS{{\em Physica}}
\def\NPA{{\em Nucl. Phys.} A}
\def\MATH{{\em J. Math. Phys.}}
\def\PRO{{\em Prog. Theor. Phys.}}
\def\NPB{{\em Nucl. Phys.} B}
\def\PLA{{\em Phys. Lett.} A}
\def\PLB{{\em Phys. Lett.} B}
\def\PLD{{\em Phys. Lett.} D}
\def\PL{{\em Phys. Lett.}}
\def\PRL{\em Phys. Rev. Lett.}
\def\PREV{\em Phys. Rev.}
\def\PREP{\em Phys. Rep.}
\def\PRA{{\em Phys. Rev.} A}
\def\PRD{{\em Phys. Rev.} D}
\def\PRC{{\em Phys. Rev.} C}
\def\PRB{{\em Phys. Rev.} B}
\def\ZPC{{\em Z. Phys.} C}
\def\ZPA{{\em Z. Phys.} A}
\def\ANNP{\em Ann. Phys. (N.Y.)}
\def\RMP{{\em Rev. Mod. Phys.}}
\def\CHEM{{\em J. Chem. Phys.}}
\def\INT{{\em Int. J. Mod. Phys.} E}
\def\NIMA{{\em Nucl. Instr. and Meth.} A}
\def\ARNS{{\em Annu. Rev. Nucl. Sci.}}
\def\FBS{{\em Few-Body Sys.}}
\def\r{\vec r}
\def\R{\vec R}
\def\p{\vec p}
\def\P{\vec P}
\def\q{\vec q}
\def\ss{\mbox{\boldmath $\sigma$}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Newcommand definitions...
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}
\newcommand{\OneStar}{$*$}
\newcommand{\TwoStar}{$*$$*$}
\newcommand{\ThreeStar}{$*$$*$$*$}
\newcommand{\FourStar}{$*$$*$$*$$*$}
\newcommand{\obs}[1]{\textcolor{red}{\mathbf{#1}}}
\newcommand{\linpol}{P_L^{\gamma}}
\newcommand{\circpol}{P_{\odot}^{\gamma}}
\newcommand{\tarpol}{P^T}
\newcommand{\recpol}{P^R}

\newcommand{\lum}{{\cal L}}
\newcommand{\sett}{{\cal S}}
\newcommand{\eff}{\varepsilon}

% \newcommand{\obs}[1]{\mathbf{#1}}
% \newcommand{\xmark}{\ding{53}}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Formatting...
\topmargin-2.8cm
\oddsidemargin-1cm
\evensidemargin-1cm
\textwidth18.5cm
\textheight25.0cm
\aboverulesep=0ex
\belowrulesep=0ex

% For fancyverbatim...
% \fvset{fontsize=\normalsize}

% formatting of tables...
\newcolumntype{R}{@{\extracolsep{1cm}}X@{\extracolsep{0pt}}}%
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{L}[1]{>{\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{Q}[1]{>{\raggedleft\arraybackslash}p{#1}} 
\newcounter{exno}
\renewcommand{\arraystretch}{1.5}  

% Set up the images/graphics package
% \setkeys{Gin}{width=\linewidth,totalheight=\textheight,keepaspectratio}
% \graphicspath{{graphics/}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%EOF

==> Photo production reactions and baryon spectroscopy/ps-cross-section.tex <==




\begin{longtable}{L{5cm} C{1cm} p{9.5cm} >{(\refstepcounter{subexno}\theexno)} C{1cm}}\label{eq:xsec}

$\obs{d\sigma^{B,T,R}}(\vec{P^\gamma},\vec{P^T},\vec{P^R},\phi)$  
& $=$ 
&
$\frac{1}{2} \left\{ \obs{d\sigma_0} \left[ 1 - \linpol \tarpol_y \recpol_{y^\prime} \cos2(\alpha - \phi) \right] \right.$
& \label{eqn:cs1} \\ 
Single spin observables 
& &
$ \quad + \obs{\Sigma} \left [- \linpol \cos2(\alpha - \phi)  + \tarpol_y \recpol_{y^\prime}   \right]$ & \label{eqn:cs2}  \\
& &
$ \quad + \obs{T} \left[ \tarpol_y - \linpol \recpol_{y^\prime} \cos 2(\alpha - \phi) \right]$ & \label{eqn:cs3}  \\
& &
$ \quad + \obs{P} \left[ \recpol_{y^\prime} - \linpol \tarpol_y \cos 2(\alpha - \phi) \right]$  & \label{eqn:cs4} 
\\
Beam-Target observables
& &
$ \quad + \obs{E} \left[ -\circpol \tarpol_z + \linpol \tarpol_x \recpol_{y^\prime}\sin2(\alpha - \phi) \right]$ & \label{eqn:cs5} \\ 
& &
$ \quad + \obs{G} \left[ \linpol \tarpol_z \sin2(\alpha - \phi) + \circpol \tarpol_x \recpol_{y^\prime} \right]$ & \label{eqn:cs6} \\  
& & 
$ \quad + \obs{F} \left[ \circpol \tarpol_x + \linpol \tarpol_z \recpol_{y^\prime} \sin2(\alpha - \phi) \right]$ & \label{eqn:cs7} \\
& & 
$ \quad + \obs{H} \left[ \linpol \tarpol_x \sin2(\alpha - \phi) - \circpol \tarpol_x \recpol_{y^\prime} \right]$ & \label{eqn:cs8} 
\\
Beam-Recoil observables
& & 
$ \quad + \obs{C_{x^\prime}} \left[ \circpol \recpol_{x^\prime} - \linpol \tarpol_y \recpol_{z^\prime} \sin2(\alpha - \phi) \right]$ & \label{eqn:cs9} \\
& & 
$ \quad + \obs{C_{z^\prime}} \left[ \circpol \recpol_{z^\prime} - \linpol \tarpol_y \recpol_{x^\prime} \sin2(\alpha - \phi) \right]$ & \label{eqn:cs10} \\
& &
$ \quad + \obs{O_{x^\prime}} \left[ \linpol \recpol_{x^\prime} \sin2(\alpha - \phi) + \circpol \tarpol_y \recpol_{z^\prime} \right]$ & \label{eqn:cs11} \\
& & 
$ \quad + \obs{O_{z^\prime}} \left[ \linpol \recpol_{z^\prime} \sin2(\alpha - \phi) - \circpol \tarpol_y \recpol_{x^\prime} \right]$ & \label{eqn:cs12} 
\\
Target-Recoil observables
& &
$ \quad + \obs{L_{x^\prime}} \left[ \tarpol_z \recpol_{x^\prime} + \linpol \tarpol_x \recpol_{z^\prime}
\cos2(\alpha - \phi) \right]$ & \label{eqn:cs13} \\
& & 
$ \quad + \obs{L_{z^\prime}} \left[ \tarpol_z \recpol_{z^\prime} - \linpol \tarpol_x \recpol_{x^\prime}
\cos2(\alpha - \phi) \right]$ & \label{eqn:cs14} \\
& &
$ \quad + \obs{T_{x^\prime}} \left[ \tarpol_x \recpol_{x^\prime} + \linpol \tarpol_z \recpol_{z^\prime}
\cos2(\alpha - \phi) \right]$ & \label{eqn:cs15} \\
& &
$ \left. \quad + \obs{T_{z^\prime}} \left[ \tarpol_x \recpol_{z^\prime} - \linpol \tarpol_z \recpol_{x^\prime}
\cos2(\alpha - \phi) \right] \right\}$ & \label{eqn:cs16} 
\\
\end{longtable}
